ACL-SPC: Adaptive Closed-Loop system for Self-Supervised Point Cloud Completion

Point cloud completion addresses filling in the missing parts of a partial point cloud obtained from depth sensors and generating a complete point cloud. Although there has been steep progress in the supervised methods on the synthetic point cloud completion task, it is hardly applicable in real-world scenarios due to the domain gap between the synthetic and real-world datasets or the requirement of prior information. To overcome these limitations, we propose a novel self-supervised framework ACL-SPC for point cloud completion to train and test on the same data. ACL-SPC takes a single partial input and attempts to output the complete point cloud using an adaptive closed-loop (ACL) system that enforces the output same for the variation of an input. We evaluate our proposed ACL-SPC on various datasets to prove that it can successfully learn to complete a partial point cloud as the first self-supervised scheme. Results show that our method is comparable with unsupervised methods and achieves superior performance on the real-world dataset compared to the supervised methods trained on the synthetic dataset. Extensive experiments justify the necessity of self-supervised learning and the effectiveness of our proposed method for the real-world point cloud completion task. The code is publicly available from https://github.com/Sangminhong/ACL-SPC_PyTorch

==> materials.tex <==
%%%%%%%%%%%%%%%% Datasets %%%%%%%%%%%%%%%%
KolektorSDD
https://www.vicos.si/resources/kolektorsdd/

DAGM2007
https://conferences.mpi-inf.mpg.de/dagm/2007/prizes.html

Severstal: Steel Defect Detection
https://www.kaggle.com/c/severstal-steel-defect-detection

%%%%% Links to some datasets
https://github.com/Charmve/Surface-Defect-Detection

%%%%%%%%%%%%%%%% Related-Papers %%%%%%%%%%%%%%%%


==> tables/ablation_loss_syn.tex <==
\begin{table}[t]
    \small
    \centering
    \subfloat[\small Effect of loss functions.]{
    \footnotesize
    \begin{tabularx}{0.55\linewidth}{l >{\centering\arraybackslash}X >{\centering\arraybackslash}X >{\centering\arraybackslash}X>{\centering\arraybackslash}X }
    \toprule
    \multirow{2}{*}{\textbf{Method}}&
    \textbf{Airplane}  & 
    \textbf{Car} &
    \textbf{Chair} 
    \\
    %\multirow{2}{*}{\textbf{Average-CD}}\\
    & P/C/CD & P/C/CD & P/C/CD
    \\
    \midrule
    - $\mathcal{L}^{wcd}$ \hspace{-10mm}
    & {1.1/18.8/19.9} 
    & {4.7/26.5/31.2}
    & {3.9/26.4/30.3}\\
    - $\mathcal{L}^{cons}$
    & {\textbf{1.1}/\hspace{1.25mm}1.1/\hspace{1.25mm}2.2} 
    & {\textbf{1.4}/\hspace{1.25mm}2.1/\hspace{1.25mm}3.6}
    & {\textbf{2.0}/\hspace{1.25mm}1.7/\hspace{1.25mm}3.7}\\
    \hspace{1mm} $\mathcal{L}^{total}$
    & {1.2/\hspace{1.25mm}\textbf{0.8}/\hspace{1.25mm}\textbf{2.0}} 
    & {1.6/\hspace{1.25mm}\textbf{1.3}/\hspace{1.25mm}\textbf{2.9}}
    & {2.2/\hspace{1.25mm}\textbf{1.5}/\hspace{1.25mm}\textbf{3.7}}\\ 
    %\midrule
    \bottomrule
    \end{tabularx}\label{tab:loss}
    }
 \hfill
    \subfloat[\small Effect of number of synthesized data.]{
    \footnotesize
    \begin{tabularx}{0.4\linewidth}{l >{\centering\arraybackslash}X >{\centering\arraybackslash}X >{\centering\arraybackslash}X>{\centering\arraybackslash}X }
    \toprule
    \multirow{2}{*}{\textbf{N}}& 
    \textbf{Airplane}  & 
    \textbf{Car} &
    \textbf{Chair} 
    \\
    & P/C/CD & P/C/CD & P/C/CD\\
    \midrule
    \vspace{0.7mm}
    {1}& {1.2/0.9/2.0} & {1.6/1.3/2.9} & {2.4/1.5/3.8}  \\ 
    {4} & {1.2/0.8/2.0} & {1.6/0.3/2.9} & {2.6/1.4/4.0}   \\
    {8} & {1.2/0.8/2.0} & {1.7/0.3/2.9} & {2.3/1.5/3.7} \\ 
    %\midrule
    \bottomrule
    \end{tabularx}\label{tab:syn}
    }
    %\vspace{-2mm}
    \caption{
        \textbf{}Ablation study on number of synthetic datas.}
        %
    
    
    \vspace{-4mm}
\end{table}

==> tables/ablation_view_multi.tex <==
\begin{table*}[t]
    \small
    \centering
    \subfloat[\small Training on single-class and multi-class.]{
    \footnotesize
    \begin{tabularx}{0.48\linewidth}{l >{\centering\arraybackslash}X >{\centering\arraybackslash}X >{\centering\arraybackslash}X>{\centering\arraybackslash}X }
    \toprule
    \multirow{2}{*}{\textbf{Class}}&
    \textbf{Airplane}  & 
    \textbf{Car} &
    \textbf{Chair} 
    \\
    & P/C/CD & P/C/CD & P/C/CD\\
    \midrule
    {Single} &  {1.2/0.8/2.0} & {1.7/1.3/2.9} & {2.3/1.5/3.7}  \\
    {Multi} & {1.4/0.8/2.2} & {1.7/1.3/2.9} & {2.5/1.4/3.9}   \\
    %\midrule
    \bottomrule
    \end{tabularx}\label{tab:class}
    }
 \hfill
    \subfloat[\small Training with single-view and multi-view.]{
    \footnotesize
    \begin{tabularx}{0.48\linewidth}{l >{\centering\arraybackslash}X >{\centering\arraybackslash}X >{\centering\arraybackslash}X>{\centering\arraybackslash}X }
    \toprule
    \multirow{2}{*}{\textbf{View}}& 
    \textbf{Airplane}  & 
    \textbf{Car} &
    \textbf{Chair} 
    \\
    & P/C/CD & P/C/CD & P/C/CD\\
    \midrule
    {1} & {1.2/0.9/2.1} & {1.6/1.3/2.9} & {2.2/1.5/3.7}  \\ 
    {5} & {1.2/0.8/2.0} & {1.7/1.3/2.9} & {2.3/1.5/3.7}   \\
    %\midrule
    \bottomrule
    \end{tabularx}\label{tab:view}
    }
    \vspace{-2mm}
    \caption{
        \textbf{}Ablation study for comparing training on multi-class, single-class, multi-view, and single-class.}
        %
    
    
    \vspace{-4mm}
\end{table*}
